Beyond Fine-Tuning: A Systematic Study of Sampling Techniques in Personalized Image Generation

Personalized text-to-image generation aims to create images tailored to user-defined concepts and textual descriptions. Balancing the fidelity of the learned concept with its ability for generation in various contexts presents a significant challenge. Existing methods often address this through diverse fine-tuning parameterizations and improved sampling strategies that integrate superclass trajectories during the diffusion process. While improved sampling offers a cost-effective, training-free solution for enhancing fine-tuned models, systematic analyses of these methods remain limited. Current approaches typically tie sampling strategies with fixed fine-tuning configurations, making it difficult to isolate their impact on generation outcomes. To address this issue, we systematically analyze sampling strategies beyond fine-tuning, exploring the impact of concept and superclass trajectories on the results. Building on this analysis, we propose a decision framework evaluating text alignment, computational constraints, and fidelity objectives to guide strategy selection. It integrates with diverse architectures and training approaches, systematically optimizing concept preservation, prompt adherence, and resource efficiency. The source code can be found at https://github.com/ControlGenAI/PersonGenSampler.

==> sections/02_related_work.tex <==
\section{Related Work} \label{sec:related_work}
\textbf{Personalized Generation} 
Due to the considerable success of large text-to-image models \cite{ramesh2022hierarchical, ramesh2021zero, saharia2022photorealistic, rombach2022high}, the field of personalized generation has been actively developed. The challenge is to customise a text-to-image model to generate specific concepts that are specified using several input images. Many different approaches \cite{DB, TI, CD, svdiff, ortogonal, profusion, elite, r1e} have been proposed to solve this problem and they can be divided into the following groups: pseudo-token optimisation \cite{TI, profusion, disenbooth, r1e}, diffusion fune-tuning \cite{DB, CD, profusion}, and encoder-based \cite{elite}. The pseudo-token paradigm adjusts the text encoder to convert the concept token into the proper embedding for the diffusion model. Such embedding can be optimized directly \cite{TI, r1e} or can be generated by other neural networks \cite{disenbooth, profusion}. Such approaches usually require a small number of parameters to optimise but lose the visual features of the target concept. Diffusion fine-tuning based methods optimise almost all \cite{DB} or parts \cite{CD} of the model to reconstruct the training images of the concept. This allows to learn the input concept with high accuracy, but the model due to overfitting may lose the ability to edit it when generated with different text prompts. To reduce overfitting and the memory used, different lightweight parameterizations \cite{svdiff, r1e, lora} have been proposed that preserve edibility but at the cost of degrading concept fidelity. Encoder-based methods \cite{elite} allow one forward pass of an encoder that has been trained on a large dataset of many different objects to embed the input concept. This dramatically speeds up the process of learning a new concept and such a model is highly editable, but the quality of recovering concept details may be low. Generally, the main problem with existing personalised generation approaches is that they struggle to simultaneously recover a concept with high quality and generate it in a variety of scenes.

\textbf{Sampling strategies}
Much work has been devoted to the study of sampling for text-to-image diffusion models, not only in the task of personalised generation, but also in image editing. In this paper, we investigate a narrower question: how we can optimally combine the two trajectories on superclass and concept to simultaneously have high concept fidelity and high editability. The ProFusion paper \cite{profusion} considered one way of combining these trajectories (mixed sampling), which we analyse in detail in our paper (see Section \ref{sec:mixed_sampling}), and show its properties and problems. In ProFusion, authors additionally proposed a more complex sampling procedure, which we observed to be redundant compared to mixed sampling, as can be seen in our experiments (see Section \ref{sec:experiments}). In Photoswap \cite{photoswap} authors consider another way of combining trajectories by superclass and concept, which turns out to be almost identical to the switching sampling strategy that we discuss in detail in Section \ref{sec:switching_sampling}. We show why this strategy fails to achieve simultaneous improvements in concept reconstruction and editability. In the paper, we propose a more efficient way of combining these two trajectories that achieves an optimal balance between the two key features of personalised generation: concept reconstruction and its editability.


==> sections/05_experiments_framework.tex <==
\textbf{A framework for selecting sampling method}
In this section, we provide an overall analysis of the performance of different sampling methods in terms of concept fidelity, alignment with a text prompt, and computational efficiency. In our conclusions, we rely mainly on the results of the user study, as current studies show that the CLIP metrics do not always match human perception. In case the user study doesn't reveal the difference between the performance of different methods, we draw conclusions based on the metrics and visual examples.

According to the Figure~\ref{fig:examples} Base sampling sometimes fails to align well with the text prompt. Fortunately, there are alternative sampling methods that can enhance text similarity. 

% здесь проблема что у нас и base comparable, при этом ему мы очень значительно по IS проигрываем, выходит что мы ничего не улучшаем? По картинкам улучшаем поэтому ссылаюсь на них

% As the user study and CLIP-metrics show Mixed, Switching, Multi-stage, and Masked sampling show comparable performance in terms of text similarity. The simplest and most cost-effective option is Switching sampling. This method increases text similarity without adding to the computational load. However, sometimes it can compromise the preservation of concepts. 
As shown by the user study and CLIP metrics, Mixed, Switching, Multi-stage, and Masked sampling achieve comparable performance in terms of TS. Among these, Switching sampling is the simplest and most cost-effective option. It improves TS without increasing computational load but may occasionally compromise concept preservation.

% Mixed Sampling addresses this issue more effectively and generally provides stable results while maintaining both concept and context (see Figure~\ref{fig:examples}). The trade-off is that it requires double the batch size compared to Switching Sampling. 
Mixed Sampling addresses this issue more effectively, generally providing stable results while preserving both concept and context (Figures~\ref{fig:examples},~\ref{fig:add_ex}). The trade-off is that it requires double the batch size compared to Switching Sampling. 

Another viable option is Masked Sampling, which can yield better concept fidelity outcomes in situations where Mixing and Switching struggle to balance context and concept. However, it demands careful tuning of hyperparameters and may produce inconsistent results because of cross-attention mask noisiness.

% Finally, ProFusion not only enhances text similarity but also preserves a high level of concept preservation (see Figure~\ref{fig:main_examples}), as indicated by user feedback. The downside is that it requires twice the U-Net inference compared to Mixed Sampling and require careful selection of many hyperparameters.
Finally, ProFusion enhances text similarity while maintaining a high level of concept preservation (Figures~\ref{fig:main_examples},~\ref{fig:add_ex_all}), as indicated by user feedback. The downside is that it requires twice the U-Net inference compared to Mixed Sampling and requires careful selection of many hyperparameters.

